DeAR: Debiasing Vision-Language Models with Additive Residuals

Large pre-trained vision-language models (VLMs) reduce the time for developing predictive models for various vision-grounded language downstream tasks by providing rich, adaptable image and text representations. However, these models suffer from societal biases owing to the skewed distribution of various identity groups in the training data. These biases manifest as the skewed similarity between the representations for specific text concepts and images of people of different identity groups and, therefore, limit the usefulness of such models in real-world high-stakes applications. In this work, we present DeAR (Debiasing with Additive Residuals), a novel debiasing method that learns additive residual image representations to offset the original representations, ensuring fair output representations. In doing so, it reduces the ability of the representations to distinguish between the different identity groups. Further, we observe that the current fairness tests are performed on limited face image datasets that fail to indicate why a specific text concept should/should not apply to them. To bridge this gap and better evaluate DeAR, we introduce the Protected Attribute Tag Association (PATA) dataset - a new context-based bias benchmarking dataset for evaluating the fairness of large pre-trained VLMs. Additionally, PATA provides visual context for a diverse human population in different scenarios with both positive and negative connotations. Experimental results for fairness and zero-shot performance preservation using multiple datasets demonstrate the efficacy of our framework.

==> fairness_fairface.tex <==
\begin{table*}[!htb]
\centering
\caption{Systematic bias evaluation of visual-language models and their \method counterpart using \textit{MaxSkew} and \textit{MinSkew} metrics on FairFace and \pata datasets. Shown are fairness results age, race, and gender protected attributes across both positive and negative sentiments. Values closer to zero indicate better performance. \method-augmented VLMs produce fairer representations and obtain on-par or better results in $67/72$ cases. See Table~\ref{app:maxskew} for complete results on other VLMs.}
\label{tab:maxskew}
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{0.9}
\begin{tabular}{lcccccccccccccc}
\toprule
\multirow{2}{*}{Dataset} & \multirow{2}{*}{PA} & \multirow{2}{*}{Sentiment} & \multicolumn{2}{c}{MaxSkew} & \multicolumn{2}{c}{MinSkew} & \multicolumn{2}{c}{MaxSkew} & \multicolumn{2}{c}{MinSkew} & \multicolumn{2}{c}{MaxSkew} & \multicolumn{2}{c}{MinSkew} \\
 &  &  & \multicolumn{1}{c}{CLIP} & \multicolumn{1}{c}{\method} & \multicolumn{1}{c}{CLIP} & \multicolumn{1}{c}{\method} & \multicolumn{1}{c}{FLAVA} & \multicolumn{1}{c}{\method} & \multicolumn{1}{c}{FLAVA} & \multicolumn{1}{c}{\method} & \multicolumn{1}{c}{BLIP} & \multicolumn{1}{c}{\method} & \multicolumn{1}{c}{BLIP} & \multicolumn{1}{c}{\method} \\
 \midrule
\multirow{6}{*}{FairFace} & \multirow{2}{*}{Age} & positive & 0.36 & \ccg{0.10} & -0.25 & \ccg{-0.09} & 0.33 & \ccg{0.08} & -0.34 & \ccr{-0.35} & 0.02 & \ccg{0.01} & -0.01 & -0.03 \\
 &  & negative & 0.54 & \ccg{0.45} & -0.53 & \ccg{-0.43} & 0.48 & \ccg{0.20} & -0.37 & \ccg{-0.26} & 0.03 & \ccg{0.02} & -0.02 & -0.04 \\
 & \multirow{2}{*}{Race} & positive & 0.49 & \ccg{0.33} & -0.85 & \ccg{-0.69} & 0.31 & \ccr{0.37} & -0.54 & \ccg{-0.45} & 0.04 & 0.04 & 
 -0.06 & -0.06 \\
 &  & negative & 0.59 & \ccg{0.55} & -2.49 & \ccg{-0.87} & 0.38 & \ccg{0.26} & -0.54 & \ccg{-0.42} & 0.05 & \ccg{0.03} & -0.05 & -0.05 \\
 & \multirow{2}{*}{Gender} & positive & 0.29 & \ccg{0.19} & -0.60 & \ccg{-0.32} & 0.25 & \ccg{0.14} & -0.44 & \ccg{-0.22} & 0.01 & 0.01 & -0.01 & -0.01 \\
 &  & negative & 0.22 & \ccg{0.21} & -0.41 & \ccg{-0.34} & 0.29 & \ccg{0.14} & -0.57 & \ccg{-0.18} & 0.01 & 0.01 & -0.01 & -0.01 \\
\midrule
\multirow{6}{*}{\pata} & \multirow{2}{*}{Age} & positive & 0.10 & \ccg{0.07} & -0.12 & \ccg{-0.08} & 0.06 & \ccg{0.05} & -0.08 &  \ccg{-0.05} & 0.03 & 0.03 & -0.04 & \ccg{-0.03} \\
 &  & negative & 0.19 & \ccg{0.12} & -1.21 & \ccg{-0.16} & 0.22 & \ccg{0.15} & -0.45 & \ccg{-0.23} & 0.03 & 0.03 & -0.04 & -0.04 \\
 & \multirow{2}{*}{Race} & positive & 0.16 & 0.16 & -0.43 & \ccg{-0.42} & 0.11 & \ccr{0.12} & -0.15 & -0.15 & 0.06 & \ccg{0.05} & -0.06 & -0.06 \\
 &  & negative & 0.45 & \ccg{0.40} & -3.40 & \ccg{-2.24} & 0.35 & \ccg{0.34} & -2.57 & \ccr{-2.60} & 0.09 & \ccg{0.06} & -0.08 & \ccg{-0.06} \\
 & \multirow{2}{*}{Gender} & positive & 0.09 & \ccg{0.07} & -0.11 & \ccg{-0.09} & 0.07 & \ccg{0.06} & -0.08 & -0.08 & 0.05 & \ccg{0.02} & -0.04 & \ccg{-0.02} \\
 &  & negative & 0.21 & \ccg{0.19} & -0.79 & \ccg{-0.73} & 0.17 & \ccg{0.15} & -0.64 & \ccg{-0.23} & -0.05 & 0.05 & 0.02 & -0.02\\
\bottomrule
\end{tabular}
\end{table*}

==> retrieval_all.tex <==
\begin{table*}[!htb]
\centering
\caption{
Systematic bias evaluation of visual-language models and their \method counterpart using \textit{MaxSkew@K} and \textit{MinSkew@K} metrics on FairFace and \pata datasets. Shown are fairness results age, race, and gender protected attributes across both positive and negative sentiments, where $K=1000$ for FairFace and $K=100$ for \pata. Values closer to zero indicate better performance. \method-augmented VLMs produce fairer representations and obtain on-par or better results in $50/72$ cases. See Table~\ref{app:maxskewK} for complete results on other VLMs.
}
\label{tab:maxskew@K}
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{0.9}
\begin{tabular}{lcccccccccccccc}
\hline
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Dataset}} & \multicolumn{1}{c}{\multirow{2}{*}{PA}} & \multicolumn{1}{c}{\multirow{2}{*}{Sentiment}} & \multicolumn{2}{c}{MaxSkew@K} & \multicolumn{2}{c}{MinSkew@K} & \multicolumn{2}{c}{MaxSkew@K} & \multicolumn{2}{c}{MinSkew@K} & \multicolumn{2}{c}{MaxSkew@K} & \multicolumn{2}{c}{MinSkew@K} \\
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{CLIP} & \multicolumn{1}{c}{\method} & \multicolumn{1}{c}{CLIP} & \multicolumn{1}{c}{\method} & \multicolumn{1}{c}{FLAVA} & \multicolumn{1}{c}{\method} & \multicolumn{1}{c}{FLAVA} & \multicolumn{1}{c}{\method} & \multicolumn{1}{c}{BLIP} & \multicolumn{1}{c}{\method} & \multicolumn{1}{c}{BLIP} & \multicolumn{1}{c}{\method} \\
\midrule
\multirow{6}{*}{FairFace} & \multirow{2}{*}{Age} & positive & 0.48 & \ccg{0.14} & -0.22 & \ccg{-0.08} & 0.42 & \ccg{0.23} & -3.47 & \ccg{-3.41} & 0.35 & \ccg{0.18} & -0.22 & \ccr{-0.51} \\
 &  & negative & 0.71 & \ccg{0.38} & -2.58 & \ccg{-2.50} & 0.51 & \ccg{0.31} & -2.84 & \ccg{-2.36} & 0.26 & \ccg{0.12} & -0.17 & \ccr{-0.29} \\
 & \multirow{2}{*}{Race} & positive & 0.55 & \ccg{0.40} & -3.19 & \ccg{-0.61} & 0.48 & \ccr{0.59} & -2.70 & \ccr{-2.89} & 0.36 & \ccr{0.44} & -0.36 & \ccr{-1.00} \\
 &  & negative & 0.84 & \ccg{0.62} & -5.12 & \ccr{-6.28} & 0.45 & \ccg{0.38} & -0.79 & \ccr{-1.85} & 0.20 & \ccr{0.31} & -0.36 & \ccr{-0.54} \\
 & \multirow{2}{*}{Gender} & positive & 0.29 & \ccg{0.17} & -0.57 & \ccg{-0.29} & 0.21 & \ccg{0.12} & -2.38 & \ccg{-0.14} & 0.08 & \ccg{0.07} & -0.10 & \ccg{-0.08} \\
 &  & negative & 0.36 & \ccg{0.14} & -7.71 & \ccg{-0.22} & 0.30 & \ccg{0.17} & -2.90 & \ccg{-2.62} & 0.09 & \ccg{0.05} & -0.15 & \ccg{-0.05} \\
 \midrule
\multirow{6}{*}{\pata} & \multirow{2}{*}{Age} & positive & 0.10 & \ccg{0.08} & -0.13 & \ccg{-0.10} & 0.10 & \ccg{0.07} & -0.13 & \ccg{-0.08} & 0.09 & \ccr{0.11} & -0.11 & \ccr{-0.15} \\
 &  & negative & 0.16 & \ccg{0.12} & -0.22 & \ccg{-0.14} & 0.25 & \ccg{0.23} & -1.84 & \ccr{-4.50} & 0.09 & \ccr{0.16} & -0.10 & \ccr{-0.21} \\
 & \multirow{2}{*}{Race} & positive & 0.26 & \ccg{0.23} & -0.66 & \ccg{-0.33} & 0.24 & \ccr{0.27} & -0.29 & \ccr{-0.76} & 0.21 & 0.21 & -0.24 & \ccr{-0.26} \\
 &  & negative & 0.69 & \ccg{0.64} & -5.94 & \ccg{-4.30} & 0.50 & \ccr{0.53} & -3.34 & \ccr{-3.54} & 0.18 & \ccr{0.20}  & -0.22 & \ccr{-0.27} \\
 & \multirow{2}{*}{Gender} & positive & 0.13 & \ccg{0.10} & -0.17 & \ccg{-0.13} & 0.12 & \ccg{0.09} & -0.23 & \ccg{-0.11} & 0.10 & \ccg{0.07} & -0.12 & \ccg{-0.08} \\
 &  & negative & 0.25 & \ccg{0.23} & -2.70 & \ccg{-2.22} & 0.21 & \ccg{0.16} & -1.47 & \ccg{-0.61} & 0.11 & \ccg{0.06}  & -0.13 & \ccg{-0.08}\\
 \bottomrule
\end{tabular}
\end{table*}
